A Proof of the Tree of Shapes in n-D

In this paper, we prove that the self-dual morphological hierarchical structure computed on a n-D gray-level wellcomposed image u by the algorithm of G{\'e}raud et al. [1] is exactly the mathematical structure defined to be the tree of shape of u in Najman et al [2]. We recall that this algorithm is in quasi-linear time and thus considered to be optimal. The tree of shapes leads to many applications in mathematical morphology and in image processing like grain filtering, shapings, image segmentation, and so on.

==> code.tex <==

\begin{algorithm}
\caption{Union-Find Algorithm (2nd pass).}
  \label{alg:union.find}
\medskip

\findroot($\zpar, x$) : P
\lcomment{modify \zpar}\;
\Begin{
  \If{\zpar(x) = x}{
    \return $x$
  }
  \Else{
    $\zpar(x) \setto \findroot(\zpar, \zpar(x))$ \rcomment{compression}\;
    \return $\zpar(x)$
  }
} %
\bigskip

\dounion($p', \, r'$) \;
\lcomment{modify \zpar, \rank, and \last}\;
\Begin{
  \If{$\rank(p') > \rank(r')$}{
    \lcomment{new root is $p'$}\;
    $\zpar(r') \setto p'$\;
    \If{$\last(r') < \last(p')$}{
      $\last(p') \setto \last(r')$
    }
  }
  \Else{
    \lcomment{new root is $r'$}\;
    $\zpar(p') \setto r'$\;
    \If{$\last(p') < \last(r')$}{
      $\last(r') \setto \last(p')$
    }
    \If{$\rank(p') = \rank(r')$}{
      $\rank(r') \setto \rank(r')+1$
    }
  }
} %
\bigskip

\unionfind(\Rel) : T \;
\lcomment{with balancing}\;
\Begin{
  \ForAll{p}{
    $\zpar(p) \setto \undef$\;
    $\rank(p) \setto 0$
  }
  \For{$i \setto N-1$ \forto 0}{
    $p \setto \Rel[i]$  \rcomment{$p$ goes from leaves to root}\;
    $\parent(p) \setto p$\;
    $\zpar(p) \setto p$\;
    $\last(p) \setto i$\;
    \ForAll{$n \in \mathcal{N}(p) \suchas \zpar(n) \neq \undef$}{
      $p' \setto \findroot(\zpar, p)$\;
      $r' \setto \findroot(\zpar, n)$\;
      \If{$r' \neq p'$}{
        $r \setto \Rel[\,last(r')\,]$\;
        $\parent(r) \setto p$\;
        $\dounion(p', r')$  \rcomment{update \zpar}\;
      }
    }
  }
  \lcomment{deallocate \zpar, \rank, and \last}\;
  \return \parent
} %
\medskip
\end{algorithm}


\begin{algorithm}
  \caption{Sort Algorithm (1st pass).}
  \label{alg:sort.algorithm}
\medskip

\ppush($q, \, h, \, U, \, \lcur$)\;
\lcomment{modify $q$}\;
\Begin{
  $[\ilower,\,\iupper] \setto U(h)$\;
  \If{$\ilower > \lcur$}{
    $\lcur' \setto \ilower$\;
  }
  \ElseIf{$\iupper < \lcur$}{
    $\lcur' \setto \iupper$\;
  }
  \Else{
    $\lcur' \setto \lcur$\;
  }
  $\push(q[\lcur'], h)$\;
} %
\bigskip

\ppop(q, \, \lcur) : H \;
\lcomment{modify $q$, and sometimes $\ell$}\;
\Begin{
  \If{$q[\lcur]$ \textup{is empty}}{
    $\lcur' \setto$ level next to \lcur such as $q[\lcur']$ is not empty\;
    $\lcur \setto \lcur'$\;
  }
  \return $\pop(q[\lcur])$\;
} %
\bigskip

\sort($U$) : Pair(Array[H], Image) \;
\Begin{
  \ForAll{h}{
    $\dejavu(h) \setto \false$\;
  }
  $i \setto 0$\;
  $\push(q[\linfty],\, \pinfty)$\;
  $\dejavu(\pinfty) \setto \true$\;
  $\lcur \setto \linfty$    \rcomment{start from root level} \;
  \While{$q$ is not empty}{
    $h \setto \ppop(q, \, \lcur)$\;
    $u^\flat(h) \setto \lcur$\;
    $\Rel[i] \setto h$\;
    \ForAll{$n \in \mathcal{N}(h) \suchas \dejavu(n) = \false$}{
      $\ppush(q,\, n,\, U, \, \lcur)$\;
      $\dejavu(n) \setto \true$\;
    }
    $i \setto i + 1$\;
    \lcomment{if $q[\lcur]$ is empty we are done with level \lcur}\;
  } %
  \return (\Rel, $u^\flat$)
} %
\medskip
\end{algorithm}




\begin{algorithm}
  \caption{ToS Computation Algorithm.}
  \label{alg:tos.algorithm}
\medskip

\canonicalizetree($f, \, \Rel, \, \parent$) \;
\lcomment{modify \parent}\;
\Begin{
  \For{$i \setto 0$ \forto $N-1$}{
    $p \setto \Rel[i]$  \rcomment{$p$ goes from root to leaves}\;
    $q \setto \parent(p)$\;
    \If{f(\parent(q)) = f(q)}{
      $\parent(p) \setto \parent(q)$
    }
  }
} %
\bigskip

\computetos($u$) : Pair(Array[P], T) \;
\Begin{
  $U$ \setto \interpolate($u$)\;
  (\Rel, $u^\flat$) \setto \sort($U$) \rcomment{1st pass}\;
  \parent \setto \unionfind(\Rel) \rcomment{2nd pass}\;
  \canonicalizetree($u^\flat$, \Rel, \parent)\;
  \return \uninterpolate(\Rel, \parent)\;
} %
\medskip
\end{algorithm}


